An inverse of Furstenberg's correspondence principle and applications to van der Corput sets

We obtain an inverse of Furstenberg's correspondence principle in the setting of countable cancellative, amenable semigroups. Besides being of intrinsic interest on its own, this result allows us to answer a variety of questions concerning sets of recurrence and van der Corput (vdC) sets, which were posed by Bergelson and Lesigne \cite{BL}, Bergelson and Ferr\'e Moragues \cite{BF}, Kelly and L\^e \cite{KL}, and Moreira \cite{Mor}. We also prove a spectral characterization of vdC sets and prove some of their basic properties in the context of countable amenable groups. Several results in this article were independently found by Sohail Farhangi and Robin Tucker-Drob, see \cite{FT}.

==> Semigroups.tex <==
\section{Extending m.p.s. from semigroups to groups}
\label{SecSemigroups}



Throughout this section we fix a countable, (left) amenable, (two-sided) cancellative, semigroup $S$ (see \Cref{DefSemigroupProps}). Statements similar to \ref{SemisImbedInGroups} were obtained, with different proofs, in \cite[Theorem 2.12]{BDM} and \cite[Corollary 2.12]{DFG}.

\begin{prop}
\label{SemisImbedInGroups}
There is a countable amenable group $G$ and an injective homomorphism $\varphi:S\to G$ such that $S':=\varphi(S)$ is a set of generators of $G$ and for any finite subset $F$ of $G$, $\bigcap_{x\in F}xS'$ is nonempty.
\end{prop}



\begin{proof}
Let $\mu:\mathcal{P}(S)\to[0,1]$ be a left invariant mean on $S$, and consider the following quotient set
\begin{equation*}
\tilde{G}=\frac{\{f:S_1\to S_2;S_1,S_2\subseteq S,\mu(S_1)=\mu(S_2)=1,f\textup{ is a $\mu$-preserving bijection}\}}{f\sim g\textup{ if }\;\exists X\subseteq S\textup{ such that }\mu(X)=1\textup{ and }f(x)=g(x)\forall x\in X}.
\end{equation*}
It is routine to check that $\tilde{G}$ is a group with the composition operation. Moreover, as $S$ is cancellative, the left translations $L_s:S\to sS;x\mapsto sx$ are elements of $\tilde{G}$ and the homomorphism $\varphi:S\to\tilde{G};s\mapsto L_s$ is injective. 
We then let $G$ be the subgroup of $\tilde{G}$ generated by $S$ (from now we consider $S$ as a subset of $G$). The group $G$ is amenable: let us check that the measure $\mu_G:\mathcal{P}(G)\to[0,1]$; $\mu_G(X)=\mu(X\cap S)$ is 
left-invariant. Firstly, for any $s\in S$ and $A\subseteq G$, 
\begin{equation*}
\mu_G(s^{-1}A)
=
\mu(s^{-1}A\cap S)
=\mu(s^{-1}(A\cap S)\cap S)
=\mu(A\cap S)
=\mu_G(A)
\end{equation*}
So $\mu_G$ is invariant by the bijections $x\mapsto s^{-1}x$, and thus by their inverses $x\mapsto sx$. As $S$ generates $G$ as a group, the measure $\mu_G$ is left-invariant in $G$. Finally, if $F\subseteq G$ is finite, we have $\mu_G\left(\cap_{x\in F}xS\right)=1$, so $\cap_{x\in F}xS$ is nonempty.
\end{proof}

In the following we let $G\supseteq S$ be the group defined in \Cref{SemisImbedInGroups}. 
\begin{comment}
\begin{notation}[Cf. {\cite[Chapter V, Definitions 2.1,2.2]{Par}}]

We say that a measure space $(X,\mathcal{B})$ is a standard Borel space when there is a complete, separable metric space $Y$, with Borel $\sigma$-algebra $\mathcal{B}_Y$, such that the $\sigma$-algebras $\mathcal{B}$ and $\mathcal{B}_Y$ are isomorphic. An \textit{atom} of a measurable space $(X,\mathcal{B})$ is a set $A_0\in\mathcal{B}$ such that the only sets $A\in\mathcal{B}$ such that $A\subseteq A_0$ are $A_0$ and $\varnothing$.
\end{notation}


\begin{theorem}
Let $(X,\mathcal{B},\mu,(T_s)_{s\in S})$ be a m.p.s. where $(X,\mathcal{B})$ is a standard Borel space and $\mathcal{B}$ is the Borel $\sigma$-algebra. Then there is an m.p.s. $(Y,\mathcal{C},\nu,(U_g)_{g\in G})$ and a measure preserving map $\pi:Y\to X$ such that $\pi\circ S_s=T_s\circ\pi$ for all $s\in S$.
\end{theorem}

\begin{proof}
We start by defining the space $Y$ and the $\sigma$-algebra $\mathcal{C}$:
\begin{gather*}
Y=\left\{(x_g)_{g\in G}\in X^G;T_sx_g=x_{sg}\textup{ for all }s\in S,g\in G\right\},\\
U_h:Y\to Y;(x_g)_{g\in G}\mapsto(x_{gh})_{g\in G},\textup{ for all }h\in G,\\
\pi_h:Y\to X;(x_g)_{g\in G}\mapsto x_h,\textup{ for all }h\in G,\\
A_h:=\{(x_g)\in Y;x_h\in A\},\textup{ for all }h\in G,A\in\mathcal{B},\\
\mathcal{C}_h=\{A_h;A\in\mathcal{B}\},\textup{ for all }h\in G,\\
\mathcal{C}=\cup_{h\in G}\mathcal{C}_h.
\end{gather*}
Note that, for all $h\in G$, $(Y,\mathcal{C}_h)$ is a standard Borel space, as the map $\pi_h:Y\to X$ gives an isomorphism from $\mathcal{C}_h$ to $\mathcal{B}$ \red{Ah wait, no. We would have to use that $\pi$ is surjective, which it need not be, as the maps $T_s$ need not be surjective (the image $T_s(X)$ need not even be Borel, it is analytic though).}
\end{proof}
\end{comment}
We start with the case in which the semigroup action is by continuous maps.

\begin{theorem}
\label{ExtendingActionsToGroups}
Let $(X,\mathcal{B},\mu,(T_s)_{s\in S})$ be a m.p.s. where $X$ is a compact metric space, $\mathcal{B}$ is the Borel $\sigma$-algebra and $T_s:X\to X$ is continuous for all $s\in S$. Then there is an m.p.s. $(Y,\mathcal{C},\nu,(U_g)_{g\in G})$ and a measure preserving map $\pi:Y\to X$ such that $\pi\circ S_s=T_s\circ\pi$ for all $s\in S$.
\end{theorem}

\begin{remark}
Even if $X$ is not a compact metric space and the maps $T_s$ are not continuous we can still use \Cref{ExtendingActionsToGroups} for most purposes, as shown in the proof of \Cref{IFCSemigroups}. However, the construction from the proof of \Cref{ExtendingActionsToGroups} need not work for an arbitrary measure space: even when $S=\mathbb{N}$, the space $Y$ defined below can be empty in pathological cases.
\end{remark}


\begin{proof}
We may assume that $T_s$ is surjective for all $s$ (if not, consider instead of $X$ the support $X_0\subseteq X$ of $\mu$. The fact that the maps $T_s$ are continuous and measure preserving implies that $T_s(X_0)$ is exactly $X_0$ for all $s\in S$). We will let
\begin{equation*}
Y=\left\{(x_g)_{g\in G}\in X^G;T_sx_g=x_{sg}\textup{ for all }s\in S,g\in G\right\}
\end{equation*}
Let $\pi:Y\to X;(x_g)\mapsto x_e$, where $e$ is the identity in $G$. The $\sigma$-algebra $\mathcal{C}\subseteq\mathcal{P}(Y)$ will be the one generated by the collection $\mathcal{C}_0$ sets of the form $A_h=\{(x_g)\in Y;x_h\in A\}$, where $h\in G$ and $A\in\mathcal{B}$. And the action $U=(U_h)_{h\in G}$ on $Y$ will be given by $U_h(x_g)_{g\in G}=(x_{gh})_{g\in G}$. 
Note that for all $h,h'\in G$, $U_h\circ U_{h'}=U_{hh'}$ and $U_h:Y\to Y$ is a measurable bijection, with $U_a^{-1}(A_h)=A_{ha}$ for $A\in\mathcal{B}$ and $a,h\in G$. Moreover, $\pi$ is also measurable.

\begin{lema}
\label{PiSurjects}
The map $\pi$ is surjective.
\end{lema}
\begin{proof}
Let $s_1\in S$ and let $(g_n)_{n\in\mathbb{N}}$ be a list of all the elements of $G$. For $n\geq1$ let $s_{n+1}$ be an element of the nonempty set $s_nS\cap g_n^{-1}S$, so that $g_n\in Ss_{n+1}^{-1}$ and $Ss_n^{-1}\subseteq Ss_{n+1}^{-1}$. Then we have $Ss_1^{-1}\supseteq Ss_2^{-1}\supseteq Ss_3^{-1}\cdots$ and $G=\cup_nSs_n^{-1}$. Now let $x_0\in X$ be arbitrary. Consider for each $n=1,2,\dots$ the sequences $(T_{gs_n}x_n)_{g\in Ss_n^{-1}}$, where $x_n\in X$ satisfies $T_{s_1}x_1=x_0$ and $T_{s_n^{-1}s_{n+1}}x_{n+1}=x_n$. Then the sequence $(x_g)_{g\in G}$ given by $x_g=T_{gs_n}x_n$ for all $s\in Ss_{n}^{-1}$ is well defined, an element of $Y$, and $\pi((x_g))=x_0$.
\end{proof}

Next we will construct the measure $\nu$. We first check that $\mathcal{C}_0\subseteq\mathcal{P}(Y)$ is an algebra. Clearly complements of sets in $\mathcal{C}_0$ are in $\mathcal{C}_0$; we now prove that the intersection of two elements of $\mathcal{C}_0$ is in $\mathcal{C}_0$ (the proof for unions is the same). First notice that for all $s\in S$ and $A_g\in\mathcal{C}_0$, 
\begin{equation}
\label{ChangeSubindex}
A_g=\{(x_h)\in Y;x_g\in A\}=\{(x_h)\in Y;x_{s^{-1}g}\in T_s^{-1}A\}=(T_s^{-1}A)_{s^{-1}g}.
\end{equation}
So given sets $A_c,B_d\in\mathcal{C}_0$, and expressing $g=s^{-1}a=(s')^{-1}b$ for some $g\in G$, $s,s'\in S$ (which can be done by letting $g^{-1}$ be in the nonempty set $a^{-1}S\cap b^{-1}S$), 
\begin{equation}
\label{43erfd6y}
A_c\cap B_d=(T_s^{-1}A)_g\cap(T_{s'}^{-1}B)_g=(T_s^{-1}A\cap T_{s'}^{-1}B)_g\in\mathcal{C}_0.
\end{equation}


We will define the measure $\nu$ in $\mathcal{C}_0$ by $\nu(A_g)=\mu(A)$ for all $A\in\mathcal{B},g\in G$. Let us check that the function $\nu$ is well defined. Suppose that $A_c=B_d$, and express $A_c=(T_s^{-1}A)_g$ and $B_d=(T_{s'}^{-1}A)_g$ as in \Cref{43erfd6y}. As the map $\pi\circ U_g:Y\to X;(x_h)_{h\in G}\mapsto x_g$ is surjective, we have $T_s^{-1}A=T_{s'}^{-1}B$, so $\mu(A)=\mu(T_s^{-1}A)=\mu(T_{s'}^{-1}B)=\mu(B)$.
We now check that $\nu$ is finitely additive in $\mathcal{C}_0$: letting $A_c,B_d\in\mathcal{C}_0$ be disjoint and using the notation above, 
\begin{equation*}
\nu(A_c\sqcup B_d)=
\nu
((T_s^{-1}A\sqcup T_{s'}^{-1}B)_g)
=\mu(T_s^{-1}A\sqcup T_{s'}^{-1}B)
=\mu(T_s^{-1}A)+\mu(T_{s'}^{-1}B)
=\nu(A_c)+\nu(B_d).
\end{equation*}
We will extend $\nu$ to a measure in $\mathcal{C}$ using Caratheodory's extension theorem. That is, we need to show that the measure $\nu$ is countably additive in $\mathcal{C}_0$. It will be enough (see \cite[Theorem 0.4]{Wa}) to show that if $(A_1)_{g_1}\supseteq(A_2)_{g_2}\supseteq\cdots$ are sets in $\mathcal{C}_0$ and $\cap_n(A_n)_{g_n}=\varnothing$, then $\lim_n\nu((A_n)_{g_n})=0$. 

We first note that $Y\subseteq X^G$ (where $X^G$ has the product topology) is compact. This is because $Y=\cap_{s\in S,g\in G}X_{s,g}$, where $X_{s,g}:=\{(x_g)\in X^G;T_sx_g=x_{sg}\}$ is closed in $X^G$ due to $T_s$ being continuous. 
Now, let $(A_1)_{g_1}\supseteq(A_2)_{g_2}\supseteq\cdots$ in $\mathcal{C}_0$ satisfy $\cap_n(A_n)_{g_n}=\varnothing$ and fix $\varepsilon>0$. We may assume that $g_{i+1}\in S^{-1}g_i$ for all $n\in\mathbb{N}$ (if not, we can use \Cref{ChangeSubindex} to express $(A_n)_{g_n}$ as $(A_n')_{g_n'}$, where $(g_n')$ is defined recursively by choosing $g_n'\in S^{-1}g_{n-1}'\cap S^{-1}g_n$, so that $g_n(g_{n}')^{-1}\in S$, and $A_n'=T_{g_n(g_n')^{-1}}^{-1}A_n$). 
For all $n\in\mathbb{N}$ let $K_n\subseteq A_n\subseteq X$ be a compact set with $\mu(A_n\setminus K_n)<\frac{\varepsilon}{2^n}$. 
As $\cap_n(K_n)_{g_n}\subseteq\cap_n(A_n)_{g_n}=\varnothing$ and $(K_n)_{g_n}$ is compact for all $n$, there is some $N\in\mathbb{N}$ such that $\cap_{i=1}^N(K_i)_{g_i}=\varnothing$, so 
\begin{equation*}
\mu(A_N)=\mu(\cap_{i=1}^NA_i)\leq\mu(\cap_{i=1}^NK_i)+\sum_{i=1}^N\mu(A_i\setminus K_i)<\varepsilon.
\end{equation*}
This implies that $\nu((A_N)_{g_N})<\varepsilon$, so $\nu((A_n)_{g_n})<\varepsilon$ for all $n\geq N$. As $\varepsilon>0$ is arbitrary, we obtain $\lim_n\nu((A_n)_{g_n})=0$, as we wanted.
\end{proof}

We can drop the condition that the maps $T_s$ are continuous for all $s\in S$ using the following result of Kuratowski:
\begin{theorem}[cf. {\cite[Corollary 3.3]{Par}}]
\label{KuratowskiThm} Let $f:X\to Y$ be an injective, Borel-measurable map between complete, separable metric spaces. Then $f(X)$ is Borel in $Y$ and $f^{-1}:f(X)\to X$ is Borel measurable.\qed
\end{theorem}

\begin{definition}
We say a measurable space $(X,\mathcal{B})$ is \textit{standard Borel} if there is a metric $d$ on $X$ such that $(X,d)$ is a complete, separable metric space with Borel $\sigma$-algebra $\mathcal{B}$. We say a m.p.s. $(X,\mathcal{B},\mu,(T_s)_{s\in S})$ is standard Borel if $(X,\mathcal{B})$ is standard Borel. 
\end{definition}

\begin{cor}
\label{ExtendingActionsToGroupsNonCont} 
Let $(X,\mathcal{B},\mu,(T_s)_{s\in S})$ be a standard Borel m.p.s. and let $G\supseteq S$ be as in \Cref{SemisImbedInGroups}. Then there is a m.p.s. $(Y,\mathcal{C},\nu,(S_g)_{g\in G})$ and a measure preserving map $\pi:Y\to X$ such that $\pi\circ S_s=T_s\circ\pi$ for all $s\in S$.
\end{cor}

\begin{proof}
We give $X$ a complete, separable metric $d$ with Borel $\sigma$-algebra $\mathcal{B}$.
Let $(A_n)_{n\in\mathbb{N}}$ be a basis of open sets of $X$, and consider the map $\Phi:X\to\{0,1\}^{S\times\mathbb{N}}$ given by $\Phi(x)=(\chi_{A_n}(T_sx))_{s\in S,n\in\mathbb{N}}$. We consider $Z:=\{0,1\}^{S\times\mathbb{N}}$ as a product space, so that it is compact and metrizable, and we let $\mathcal{D}$ be its Borel $\sigma$-algebra. Note that $\Phi$ is measurable. We let $m$ be the measure in $Z$ given by $m(D)=\mu(\Phi^{-1}D)$ for all $D\in\mathcal{D}$, and we define for all $t\in S$ the (continuous) maps 
\[U_t:Z\to Z;(\varepsilon_{s,n})_{s\in S,n\in\mathbb{N}}\mapsto (\varepsilon_{st,n})_{s\in S,n\in\mathbb{N}}\] Note that $\Phi\circ T_s=U_s\circ\Phi$ for all $s\in S$, so the maps $U_s$ preserve the measure $m$.

By \Cref{ExtendingActionsToGroups} there is a m.p.s. $(Y,\mathcal{C},\nu,(S_g)_{g\in G})$ and a measure preserving map $\pi_Z:Y\to Z$ such that $\pi_Z\circ S_s=U_s\circ\pi_Z$ for all $s\in S$.

Now, as the sets $A_n$ form a basis for the topology of $X$, there cannot be two points $x,y$ such that $x\in A_n\iff y\in A_n$ for all $n\in\mathbb{N}$, meaning that the map $\Phi$ is injective. 
So by \Cref{KuratowskiThm}, $Z_0:=\Phi(X)$ is Borel in $\{0,1\}^{S\times\mathbb{N}}$, and the bijection $\Phi^{-1}:Z_0\to X$ is Borel measurable.
We have $m(Z_0)=1$, so letting $Y_0=\pi_Z^{-1}(Z_0)\subseteq Y$ and $Y_1=\cap_{g\in G}S_gY_0$, the set $Y_1$ has measure $1$
and is $G$-invariant, and the map $\pi=\Phi^{-1}\circ\pi_Z:Y_1\to X$ is measure preserving (as both $\pi_Z$ and $\Phi^{-1}$ are) and such that, for all $s\in S$, $\pi\circ S_s=T_s\circ\pi$.

\begin{center}
\begin{tikzcd}
X \arrow[d, "T_s"'] \arrow[r, "\Phi", "\cong"'] & Z_0 \arrow[d, "U_s"'] & Y_1 \arrow[d, "S_s"'] \arrow[l, "\pi_Z"'] \\
X \arrow[r, "\Phi", "\cong"']                   & Z_0                   & Y_1 \arrow[l, "\pi_Z"']   
\end{tikzcd}
\end{center}
\vspace{-20pt}\qedhere
\end{proof}


